Generic Multicast (Extended Version)

Communication primitives play a central role in modern computing. They offer a panel of reliability and ordering guarantees for messages, enabling the implementation of complex distributed interactions. In particular, atomic broadcast is a pivotal abstraction for implementing fault-tolerant distributed services. This primitive allows disseminating messages across the system in a total order. There are two group communication primitives closely related to atomic broadcast. Atomic multicast permits targeting a subset of participants, possibly stricter than the whole system. Generic broadcast leverages the semantics of messages to order them only where necessary (that is when they conflict). In this paper, we propose to combine all these primitives into a single, more general one, called generic multicast. We formally specify the guarantees offered by generic multicast and present efficient algorithms. Compared to prior works, our solutions offer appealing properties in terms of time and space complexity. In particular, when a run is conflict-free, that is no two messages conflict, a message is delivered after at most three message delays.

==> Makefile <==
ALL=$(wildcard *.tex)
BIB=$(wildcard *.bib)
MAIN=main.tex
LATEX=rubber --pdf --unsafe

.DEFAULT_GOAL := all

all: ## Build full document
	$(LATEX) $(MAIN)                # main run

clean: ## Clean LaTeX and output figure files
	rubber --clean $(MAIN)

watch: ## Recompile on any update of LaTeX or SVG sources
	@while [ 1 ]; do;          \
	  inotifywait $(ALL);    \
	  sleep 0.01;            \
          make all;              \
          echo "\n----------\n"; \
          done

help:  # http://marmelab.com/blog/2016/02/29/auto-documented-makefile.html
	@grep -P '^[a-zA-Z_-]+:.*?## .*$$' $(MAKEFILE_LIST) | sort | awk 'BEGIN {FS = ":.*?## "}; {printf "\033[36m%-20s\033[0m %s\n", $$1, $$2}'

.PHONY: help

